SciFix: Outperforming GPT3 on Scientific Factual Error Correction

Due to the prohibitively high cost of creating error correction datasets, most Factual Claim Correction methods rely on a powerful verification model to guide the correction process. This leads to a significant drop in performance in domains like scientific claims, where good verification models do not always exist. In this work, we introduce SciFix, a scientific claim correction system that does not require a verifier but can outperform existing methods by a considerable margin -- achieving correction accuracy of 84% on the SciFact dataset, 77% on SciFact-Open and 72% on the CovidFact dataset, compared to next best accuracies of 7%, 5%, and 15% on the same datasets respectively. Our method leverages the power of prompting with LLMs during training to create a richly annotated dataset that can be used for fully supervised training and regularization. We additionally use a claim-aware decoding procedure to improve the quality of corrected claims. Our method outperforms the very LLM that was used to generate the annotated dataset -- with Few-Shot Prompting on GPT3.5 achieving 58%, 61%, and 64% on the respective datasets, a consistently lower correction accuracy, despite using nearly 800 times as many parameters as our model.

==> figtables/explanation_mistake_neurips.tex <==
\begin{figure*}
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small,frame=single]
Explanation | \textcolor{red}{Incorrect Prediction:} The evidence mentions that self-harm rates were more 
than ten times higher in female prisoners than in male inmates, hence the claim is true |
Claim: The risk of male prisoners harming themselves is ten times that of female prisoners.
\end{Verbatim}
    \caption{Explanation directly contradicts the predicted claim, signaling a mistake}
    \label{fig:explanation_mistake}
\end{figure*}

==> figtables/sari_neurips.tex <==
\begin{figure*}
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small,frame=single]
Sources: ... 
\textcolor{cyan}{References: } 40mg/day dosage of folic acid and 2mg/day dosage of vitamin B12 
\textbf{does not affect} chronic kidney disease (CDK) progression.  
\textcolor{red}{Prediction 1: } 40mg/day dosage of folic acid and 2mg/day dosage of vitamin B12 
\textbf{has an affect on} chronic kidney disease (CDK) progression.  
\textcolor{cyan}{Prediction 2: } 40mg/day dosage of folic acid and 2mg/day dosage of vitamin B12 
\textbf{has an affect on} chronic kidney disease (CDK) progression.  
            SARI 1: \textbf{92.91}      SARI 2: 75.75
\end{Verbatim}
    \caption{SARI metric is higher for an incorrect claim than a correct claim. It is unable to identify semantic similarity}
    \label{fig:sari}
\end{figure*}


==> figtables/success_neurips.tex <==
\begin{figure*}
\begin{Verbatim}[commandchars=\\\{\}, fontsize=\small,frame=single]
\textcolor{red}{Claim:} general exercise therapy is more effective than Scapular stabilizer 
exercises in reducing pain and improving function of the shoulder.
\textcolor{blue}{Proposed Correction:} Scapular stabilizer exercises are more effective than 
general exercise therapy in reducing pain and improving function of the shoulder.

\textcolor{red}{Claim:} Severe immunosuppression and also a cytokine storm characterize covid-19 
infections
\textcolor{blue}{Proposed Correction:} Severe immunosuppression and not a cytokine storm 
characterize covid-19 infections

\textcolor{red}{Claim:} APOE4 expression in iPSC-derived neurons increases AlphaBeta production and 
tau phosphorylation, delaying GABA neuron degeneration.
\textcolor{blue}{Proposed Correction:} APOE4 expression in iPSC-derived neurons increases AlphaBeta 
production and tau phosphorylation, promoting GABA neuron degeneration.

\textcolor{red}{Claim:} The most prevalent adverse events to Semaglutide are cardiovascular.
\textcolor{blue}{Proposed Correction:} The most prevalent adverse events to Semaglutide are metabolic.

\textcolor{red}{Claim:} Coronavirus vaccine to be tested on mice by june 1
\textcolor{blue}{Proposed Correction:} Coronavirus vaccine to be tested on humans by june 1

\textcolor{red}{Claim:} Uk rolls out all doses of covid-19 vaccination.
\textcolor{blue}{Proposed Correction:} Uk rolls out first doses of covid-19 vaccination
\end{Verbatim}
    \caption{Examples of the claim correction system performing well on a diverse set of input types. The system is able to swap entities, negate only specific parts of a sentence, alter numerical quantifiers in word form, and more}
    \label{fig:success}
\end{figure*}
